Double-Iterative Gaussian Process Regression for Modeling Error Compensation in Autonomous Racing

Autonomous racing control is a challenging research problem as vehicles are pushed to their limits of handling to achieve an optimal lap time; therefore, vehicles exhibit highly nonlinear and complex dynamics. Difficult-to-model effects, such as drifting, aerodynamics, chassis weight transfer, and suspension can lead to infeasible and suboptimal trajectories. While offline planning allows optimizing a full reference trajectory for the minimum lap time objective, such modeling discrepancies are particularly detrimental when using offline planning, as planning model errors compound with controller modeling errors. Gaussian Process Regression (GPR) can compensate for modeling errors. However, previous works primarily focus on modeling error in real-time control without consideration for how the model used in offline planning can affect the overall performance. In this work, we propose a double-GPR error compensation algorithm to reduce model uncertainties; specifically, we compensate both the planner's model and controller's model with two respective GPR-based error compensation functions. Furthermore, we design an iterative framework to re-collect error-rich data using the racing control system. We test our method in the high-fidelity racing simulator Gran Turismo Sport (GTS); we find that our iterative, double-GPR compensation functions improve racing performance and iteration stability in comparison to a single compensation function applied merely for real-time control.

==> sections/methods_old.tex <==
\section{Trajectory Planning and Control Algorithms}\label{Sec:Plan_MPC}
In this section, we introduce the framework planning and control framework, which consists of two modules: 1.) time-optimal trajectory planning and 2.) reference-tracking model predictive control (MPC). These algorithms were developed previously \cite{ourpriorwork}. It will serve as the base for our double-iterative GPR-based modeling error compensation work.
\subsection{Time-Optimal Trajectory Planning}\label{Sec:TrajPlan}
% \red{Based on the vehicle model given in the last section, in this section, we will introduce the time-optimal trajectory planning method proposed in our previous work \cite{}
% based on the vehicle model and the geometry of the track.}

% Since the 'time' is an implicit temporal vehicle state, we instead express it in the spacial domain related to the Frenet coordinate \cite{verschueren2014towards}\cite{chang2018near}.
% However, the nonlinear objective and vehicle model impedes the optimization; therefore some papers simplify the nonlinear objective as a near-optimal problem such as the curvature-optimal planning. In this paper, we propose a new solution using the linearized curvature-optimal planning to warm-start the nonlinear time-optimal planning. In the following subsections, we present the planning problem formulation and the optimization-based solving algorithm.

% \subsubsection{Time-optimal Planning}
% \label{SubSec:Time-optimal}

When the racing vehicle runs around a track, we can formulate the Frenet coordinate related to the track centerline as shown in Fig \ref{fig:vehicle model}. The vehicle speed projected to the centerline is defined as $\dot{s}$ in \eqref{Equ:s}.
% Then the lap time $T$ in one loop can be expressed as the integral of time 
% % differential with respect to the centerline as \eqref{Equ:TimeObj} 
% as
% \begin{align}
% \nonumber T&=\int_{0}^{T} 1 d t=\int_{s_{0}}^{s_{f}} \frac{d t}{d s} d s=\int_{s_{0}}^{s_{f}} \frac{1}{\dot{s}} d s\\
% &= \int_{s_{0}}^{s_{f}} \frac{1-\kappa(s) e_{y}}{V_{x} \cos \left(e_{\psi}\right)-V_{y} \sin \left(e_{\psi}\right)} d s
%     \label{Equ:Time3}
% \end{align}
% By discretizing the $T$, we have
% \begin{equation} \label{Equ:TimeObj}
% T = \sum_{k=1}^{N}\frac{1-\kappa(s^{k}) e^{k}_{y}}{V^{k}_{x} \cos \left(e^{k}_{\psi}\right)-V^{k}_{y} \sin \left(e^{k}_{\psi}\right)} \Delta s_k \\
% \end{equation}
The objective function of lap time can be written as 
\begin{subequations}\label{equ:24}\label{Equ:TimeObj}
    \begin{equation} \label{equ:24a}
        \min_{\{x_i\}_{i=1}^N,\{u_{i}\}_{i=1}^N} T =
    \sum_{k=1}^{N}\frac{1-\kappa(s^{k}) e^{k}_{y}}{V^{k}_{x} \cos e^{k}_{\psi}-V^{k}_{y} \sin e^{k}_{\psi}} \Delta s_k 
    \end{equation}
    \begin{equation}\label{equ:24b}
        \mathrm{ s.t. } \quad \mb{x}_{k+1}= \mb{x}_{k} + f(\mb{x}_{k},\mb{u}_{k}) \Delta t
    \end{equation}
    \begin{equation}\label{equ:24c}
        \mb{x}_{1}=\mb{x}_{N}
    \end{equation}
    \begin{equation}\label{equ:24d}
        w_{r,k} \leq e_{y,k} \leq w_{l,k}
    \end{equation}
    \begin{equation}\label{equ:24e}
        \delta_{\min,k } \leq \delta_k \leq \delta_{\max,k }
    \end{equation}
\end{subequations}

As we can see, this objective is highly nonlinear. Directly minimizing $T$ using nonlinear solver is very likely to stop at the local minima. 

% \red{To solve this problem we use a curvature-optimal as a warm-start for time-optimal planning.}
% According to \cite{}, by considering minimizing an objective function including curvature $\kappa$ as well as $V_y$ and $\dot{\delta}$

% % \begin{equation} \label{Equ:KapObj}
% % J_{\kappa}=w_{\kappa, 1}\left(\frac{\dot{\psi}}{V_{x}}\right)^{2}+w_{\kappa, 2} V_{y}^{2}+w_{\kappa, 3} \dot{\delta}
% % \end{equation}
% \begin{equation} \label{Equ:KapObj}
% J_{\kappa}=w_{\kappa, 1}\kappa^{2}+w_{\kappa, 2} V_{y}^{2}+w_{\kappa, 3} \dot{\delta}
% \end{equation}
% where 
% \begin{equation} \label{Equ:Kap}
% \kappa=\frac{d \psi}{d s}=\frac{d \psi}{d t} \frac{d t}{d s}=\frac{\dot{\psi}}{\dot{s}} \approx \frac{\dot{\psi}}{V_{x}}.
% \end{equation}

% As we can see, the object of  curvature-optimal is quadratic, 
% by iteratively optimizing the velocity and the path curvature 
% % based on the linearized vehicle model \cite{kapania2016sequential}
% , we can obtain a warm-start trajtectoy for time-optimal planning.
% For more details please refer to \cite{}.


% \subsection{Curvature-optimal Planning}
\label{SubSec:Kap-optimal}

% Inspired from \cite{kapania2016sequential}, we can simplify the time-optimal objective as a quadratic programming planning with the minimum curvature and maximum velocity. Though the solution is only near-optimal to the original nonlinear problem, we can quickly approach the global optimal and use it as a good warm-start for the nonlinear solver.

% \begin{align}
%     T= & \int_{s_{0}}^{s_{f}} \frac{1-\kappa(s) e_{y}}{V_{x} \cos \left(e_{\psi}\right)-V_{y} \sin \left(e_{\psi}\right)} d s \label{Equ:Time2} \\
%     \approx & \int_{s_{0}}^{s_{f}} \frac{d s}{V_{x}} \label{Equ:Time3}
% \end{align}

% Bringing Equ. (\ref{Equ:s}) to (\ref{Equ:TimeObj}), we derive (\ref{Equ:Time2}). Then we can simplify the objective assuming the curvature $\kappa$ and the yaw difference angle $e_\psi$ are much smaller than $1$ and derive the approximate objective (\ref{Equ:Time3}). This new objective is very straightforward that we should maximize the vehicle velocity to minimize the lap time. 

% \begin{equation} \label{Equ:MaxV}
%     V_{x,max} = \sqrt{F_{y,max}/\kappa}
% \end{equation}

% The limitations of velocity are at sharp corners where the tire friction is inadequate to provide enough turning forces. According to equ. (\ref{Equ:MaxV}), the maximum velocity is related to the lateral forces and the path curvature. By minimizing the path curvature, we can finally increase the velocity, so we derive the idea of curvature-optimal path planning.

% \begin{equation} \label{Equ:Kap}
% \kappa=\frac{d \psi}{d s}=\frac{d \psi}{d t} \frac{d t}{d s}=\frac{\dot{\psi}}{\dot{s}} \approx \frac{\dot{\psi}}{V_{x}}
% \end{equation}

% According to the definition of path curvature and applying the simplification of $\dot{s}$ again, we can obtain the new expression of $\kappa$ as Equ. (\ref{Equ:Kap}). Consequently, we can formulate the quadratic programming curvature-optimal objective as Equ. (\ref{Equ:KapObj}).

% \begin{equation} \label{Equ:KapObj}
% J_{\kappa}=w_{\kappa, 1}\left(\frac{\dot{\psi}}{V_{x}}\right)^{2}+w_{\kappa, 2} V_{y}^{2}+w_{\kappa, 3} \dot{\delta}
% \end{equation}

% where, $\frac{\dot{\psi}}{V_{x}}$ denotes the approximate curvature. In addition, we add two regularization terms of lateral and steering angle changing rate to stabilize the QP solver. 

% Finally, we can iteratively optimize the velocity and the path curvature based on the linearized vehicle model \cite{kapania2016sequential}. Since two optimization problems are only quadratic programming, we can avoid the local minima problem in the nonlinear time-optimal planning. 



\subsection{MPC Tracking Controller}
\label{Sec:Controller}

In section \ref{Sec:VehicleModel} and \ref{Sec:TrajPlan}, we formulate the vehicle model and formulate the time-optimal trajectory planning. In this section, we introduce the model predictive controller (MPC) to track reference trajectory with the vehicle model.
% Commonly, MPC for autonomous driving cars decouples the vehicle longitudinal and lateral models\cite{kong2015kinematic}, where throttle and brake pedals control the velocity and the steering wheel controls the vehicle heading, separately.
% However, the longitudinal and lateral dynamics of racing cars are tightly related when $V_y$ is large, so that the vehicle slip angle $\beta$ shown in Fig. \ref{fig:vehicle model} separate vehicle heading and the velocity direction. In addition, the throttle and brake cause weight transfer and influence the wheel load that indirectly change the maximum lateral tire friction. 
% Consequently, 
Here, we adopt the MPC with coupled longitudinal and lateral vehicle models and linearized at the reference states. Then we formulate the tracking objective and constraints for the MPC as the following:
% Besides, we apply a hyperparameter auto-tuning method to improve the performance by tuning the MPC weights.
%
% to their derivative to confine the fast changing. 
%

% \subsubsection{Objective and Constraints}
When operating the racing vehicles, we expect to minimize the error between the vehicle states and the reference trajectory. Based on that goal, we design the objective function for our MPC controller as
% At each control time step, we observe the vehicle states and find the nearest point to the reference path, deriving the reference states $x_ref$ in the Frenet coordinate. Then we interpolate the reference trajectory in the horizon to the maximum step $N_p$.

\begin{subequations}\label{Equ:MPCCons}
\begin{align} 
J_{c}=\sum_{k=1}^{N_{p}} & w_{v_{x}}\left(v_{x, k}-v_{x, k}^{\mathrm{ref}}\right)^{2}+w_{v_{y}}\left(v_{y, k}-v_{y, k}^{\mathrm{ref}}\right)^{2} \nonumber \\
&+w_{\omega}\left(\dot{\psi}_{k}-\dot{\psi}_{k}^{\mathrm{ref}}\right)^{2}+w_{e_{\psi}} e_{\psi, k}^{2} \nonumber\\
&+w_{e_{y}} e_{y, k}^{2}+w_{\dot{\delta}} \dot{\delta}_{k}^{2} \label{Equ:MPCObj}
\end{align}
% \begin{subequations}
\begin{equation}\label{Equ:MPC_equ_Constrain}
% \begin{gathered}
\text { s.t. } 
\quad \mb{x}_{k+1}=\mb{A}_{k} \mb{x}_{k}+\mb{B}_{k} \mb{u}_{k}+\mb{D}_{k} 
\end{equation}
\begin{equation}
\quad \forall k \in\left[1, \ldots, N_{p}\right] \\
\end{equation}
\begin{equation}
\quad-\delta_{\max } \leq \delta_{k} \leq \delta_{\max } \\
\end{equation}
\begin{equation}
a_{p,k, min} \leq a_{p, k} \leq a_{p, k, max} \\
\end{equation}
\begin{equation}
-\dot{\delta}_{\max } \leq \dot{\delta}_{k} \leq \dot{\delta}_{\max }
% \end{gathered}
\end{equation}
\end{subequations} where $N_p$ is the prediction horizon of MPC. 
To induce a QP problem and therefore facilitate the real-time implementation of MPC,
we linearize the vehicle model \eqref{equ:model_summary2} to formulate \eqref{Equ:MPC_equ_Constrain}.
% The vehicle model 

In the objective equation (\ref{Equ:MPCObj}), the first three terms are vehicle dynamic states errors; The fourth and fifth term are used to minimize the kinetic states error of $e_{psi}$, $e_y$, respectively. And the $\dot{\delta}$ term is used to regularize steering input. The equality constraint represents the linearized vehicle dynamics, and the inequality constraints set the limitations for vehicle control inputs.

By solving the QP problem, we can obtain the optimal tracking control input by minimizing the aforementioned tracking errors. Eventually, the vehicles can follow the reference trajectory and achieve the planned lap time.

Here we use a heuristic nominal trajectory $\bar{\mb{x}}_k$ that smoothly transits the current state to the reference trajectory as the linearization point for \eqref{Equ:MPC_equ_Constrain}
\begin{equation} \label{Eqn:refstate}
    \bar{\mb{x}}_k = \mb{x}_{k}^{ref} + \lambda_{k}(\mb{x}_0 - \mb{x}_{0}^{ref})
\end{equation}
where $\mb{x}_0$ is the current state of the vehicle; $\mb{x}_{0}^{ref}$ and $\mb{x}_{k}^{ref}$ are the reference states at the current time step and $k$ steps in the horizon. The weight sequence $\{\lambda_k\}_{k=0}^{N_p}$ is a monotonically decreasing sequence with $\lambda_0=1$ and $\lambda_{N_p}=0$. The weight sequence controls how fast $\mb{x}_k$ transits from the current state back to the reference. 
%
% At each control step, we linearize the vehicle model at the predicted states $\bar{\mb{x}}_k$ at $k$ future steps as
% \begin{equation} \label{Equ:refstate}
%     \bar{\mb{x}}_k = \mb{x}_{k,ref} + (\mb{x}_0 + \mb{x}_{0,ref})
% \end{equation}
% where, $\mb{x}_0$ denotes the current vehicle state; 
% $\mb{x}_{0,ref}$ and $\mb{x}_{k,ref}$ indicate the reference states at the current time step and $k$ steps in the horizon. 
The nominal trajectory $\bar{\mb{x}}_k$ are then applied to derive 
% then apply 
the linearized
% and discretization to the 
vehicle model  \eqref{Equ:MPC_equ_Constrain}.
% \eqref{equ:model_summary}
% to derive the linearized state space function as $\mb{x}_{k+1} = \mb{A}_k \mb{x}_k + \mb{B}_k \mb{u}_k + \mb{D}_k$.}


\section{Double Iterative GPR-based Trajectory Planning and Mode Predictive Control  Framework}\label{Sec:double_gpr_plan_mpc}
In this section, we will introduce the proposed double iterative modeling error compensation framework in the autonomous racing task.
% how do we apply GPR in both path planning and MPC. 
In this framework, we apply GPR-based error compensation model in time-optimal planning and MPC stage, respectively.
% Since 
% in this two modules, the models we use are different, 
Since we use a different linearized model for the low level-control, to better compensate for the linearization error for the MPC vehicle model, we correspondingly build two different GPR models for planning and MPC, respectively. The details of these two different GPR models will be introduced in the following sections.
% we will introduce how do we apply GPR in these two stages of task, respectively.
% In our two task, due to the different time computing requirement, the models that we use are different.
% In offline planning, the model accuracy is more important while 
% computation time cost for the optimization is not a strict requirement. 
% Therefore, a nonlinear model is adopted in offline time-optimal trajectory planning.
% In contrast, for MPC, real-time implementation is critical.
% Therefore, a linearized and discrete-time version of the model in section \ref{Sec:VehicleModel} is applied. 

% To achieve, we build different GPR model for this two task, respectively.
% Please see below

\subsection{GPR-Based Trajectory Planning}\label{Sec:gpr_plan}
For GPR-based trajectory planning, based on the time-optimal goal that we proposed in  \eqref{Equ:TimeObj}, we further proposed the constraints that after applying GPR error correction in vehicle model \eqref{equ:model_summary2} 
as
\begin{equation}
     \dot{\mb{x}} = f(\mb{x}_k,\mb{u}_k) + \boldsymbol{\mu}^{plan}(\mb{z}_k)
\end{equation}
where  $\boldsymbol{\mu}^{plan}$ is the mean of the GPR error model
\begin{equation}
\begin{aligned}
\mb{g}^{plan}(\mb{z})\sim 
\mathcal{N}(\boldsymbol{\mu}^{plan}(\mb{z}), \mb{\Sigma}^{plan}(\mb{z}))
\end{aligned}
\end{equation}

When we build or update the dataset of this GPR model. the output data point $\mb{y}_k$ in the dataset $\mathcal{D}$ of the GPR in the planning stage is calculated as

\begin{equation}
    \mb{y}_k = \dot{\mb{x}}^{real}_k - f(\mb{x}^{real}_k,\mb{u}_k),
\end{equation}
here $\dot{\mb{x}}^{real}_k$ is obtained from differentiation of the real state $\mb{x}^{real}$.

For GPR, how to select feature $\mb{z}_k$ is very important. In this work, we select the feature by calculating the correlation coefficients between state errors and some candidate features, choose the states that have the highest correlation with the state error as our feature.

% As for the feature $\mb{z_k}$ that we choose to predict the model error wiil be described in Section \ref{sec5}.

% \red{\begin{equation}
%     \hat{a}_z =  g_{a_z}(a_x, a_p, \Theta,\dot{\Theta})
% \end{equation}}


% \begin{algorithm}[ht]
% \LinesNumbered
% \SetAlgoLined
% \KwOut{Reference path, curvature and velocity} \vspace{1 mm}
%  $X^{[0]},Y^{[0]},\kappa^{[0]},x^{[0]} \xleftarrow{}$ Initialize path, curvature and other states \\[1 mm]
%  \While{$\Delta t>\varepsilon$}{
% $V_x^{[i]}$ $\xleftarrow{}$ Generate velocity profile($ \kappa^{[i-1]}, x^{[i-1]}$)\hspace{10cm} \phantom{.} \hspace{0.65cm} (Section \ref{sec:velocityprofile})\\[1 mm]
% $e_y^{[i]}, e_{\psi}^{[i]},x^{[i]} \xleftarrow{}$ $\kappa$-opt path Planning($ V_x^{[i]},x^{[i-1]}$) \hspace{10cm} \phantom{.} \hspace{1.75cm} (Section \ref{sec:k-opt path})\\[1 mm]
% $X^{[i]},Y^{[i]},\kappa^{[i]} \xleftarrow{}$ Path, curvature update($e_y^{[i]}, e_{\psi}^{[i]}$)\hspace{10cm} \phantom{.} \hspace{2.0cm} (Section \ref{sec:pathupdate})\\[1 mm]
% $t^{[i]}, \Delta t$ $\xleftarrow{}$ Compute lap time($X^{[i]},Y^{[i]},V_x^{[i]}$)\hspace{10cm} \phantom{.} \hspace{1.075cm} (Section \ref{sec:pathupdate})
%  }
%  \caption{Iterative Trajectory Planning }\label{Alg:ATP}
% \end{algorithm}


\subsection{GPR-Based MPC Tracking Controller}

Similarly, we apply the error compensation term in the MPC vehicle model constrain \eqref{Equ:MPC_equ_Constrain} as 
\begin{equation}
    % \text { s.t. } \quad 
    \mb{x}_{k+1}=\mb{A}_{k} \mb{x}_{k}+\mb{B}_{k} \mb{u}_{k}+\mb{D}_{k} + \boldsymbol{\mu}^{MPC}(\mb{z}_k) 
\end{equation}
where $\boldsymbol{\mu}^{MPC}$ is the mean of the GPR error model 
\begin{equation}
\begin{aligned}
\mb{g}^{MPC}(\mb{z})\sim 
\mathcal{N}(\boldsymbol{\mu}^{MPC}(\mb{z}), \mb{\Sigma}^{MPC}(\mb{z}))
\end{aligned}
\end{equation}

The output data point $\mb{y}^{MPC}_k$ in the dataset $\mathcal{D}$ of the GPR in the MPC stage is calculated as

\begin{equation}
\mb{y}^{MPC}_k = \mb{x}^{real}_{k+1} - (\mb{A}_{k} \mb{x}^{real}_{k}+\mb{B}_{k} \mb{u}_{k}+\mb{D}_{k}) 
\end{equation}

One thing worth noticing is that, 
in our work we assume that the feature $\mb{z}_k$ can be derived from state $\mb{x}_k$, $\mb{z}_k = h(\mb{x}_k)$.
% for a more accurate error compensation,
Here the feature $\mb{z}_k$ we use to calculate the error compensation 
is also derived from the nominal trajectory state $\mb{\bar{x}}$ 
% for linearization 
in \eqref{Eqn:refstate}, $\mb{z}_k = \mb{\bar{z}}_k = h(\mb{\bar{x}}) $. 
% therefore is a transit feature between the feature $\mb{z}_0$ based on the current state $\mb{x}_0$ and the reference feature $\mb{z}_{k,ref}$ based on reference state $\mb{x}_{k,ref}$. 


% As for how we drive $\mb{z}$ from the state $\mb{x}$, we will introduce it later in Section \ref{subsec:state_feature_select}. 

% $\dot{\mb{x}}^k_{real}$ is obtained from differentiation of the real state $\mb{x}_{real}$.

% Similar the dataset for the GPR useded in MPC task is generated by
% \begin{equation}
% \mb{y}_k = \mb{x}_{k+1} - (\mb{A}_{k} \mb{x}_{k}+\mb{B}_{k} \mb{u}_{k}+\mb{D}_{k}) 
% \end{equation}

% \red{What terms to compensate}
% Refer:
% Can we use variables to 
% Why do we add GPR on both planning and control

\subsection{Double Iterative Error Modeling Error Compensation framework}\label{subsec:framework}
Eventually, by combing GPR-based Time-Optimal Trajectory Planning and GPR-base MPC, in this section, we will introduce our framework of Double Iteartive GPR-base Error Modeling for autonomous racing. The idea is illustrated in Figure \ref{Fig:framework}.

In this framework, without enabling GPR-based modeling error compensation, we first plan a curvature-optimal trajectory (\textbf{Step (1.1)}) as a warm-start and use the MPC controller without GPR error compensation to track that curvature-optimal trajectory (\textbf{Step (2)}) to collect data. Here we count this first iteration as the 0th iteration. The reason we choose to track the curvature-optimal trajectory as a warm-start is to enrich the data diversity.
% Since GPR is very likely to overfit certain data,
Our experimental result shows that with data from tracking curvature-optimal as a warm-start instead of tracking time-optimal, the prediction performance of GPR  will increase.
%
After obtaining the first data in the 0th iteration, we will use that data to build our first GPR error compensation models (\textbf{Step (3)}) and apply them in the time-optimal trajectory planning \textbf{Step (1.2)} and MPC tracking \textbf{Step (2)}. Similarly after the 1st iteration, we collect data again and use them to update our GPR model (\textbf{Step (3)}). 
% which will be introduced later. 
With this 
% \textbf{Planning-Running-GPR Updating} 
iteration is keep increasing, we will able continuously update our GPR model and obtain GPR models that can continuously receive the most recent data that can
better predict error in both planning and tracking and therefore plan a more feasible trajectory and track the planned trajectory with better performance.
% \red{Please notice that in each following time-optimal trajectory planning, we still use the planned curvature-optimal trajectory as a warm-start.}

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{fig/framework2.png}
    \caption{
    The framework of double iterative GPR-based error compensation Trajectory Planning and Mode Predictive Control; 
    \; \textbf{(1.1)} For the \textit{0th} iteration, plan a curvature-optimal trajectory without GPR error compensation as warm-start; 
    \;\textbf{(1.2)} From the \textit{1st} iteration, plan the time-optimal trajectory with GPR error compensation;
    \;\textbf{(2)} Tracking the planning trajectory without (in the \textit{0th}iteration) / with (after the \textit{0th} iteration) GPR error compensation in MPC;
    \;\textbf{(3)} Collect data and Update GPR error compensation models.
    }
    \label{Fig:framework}
\end{figure}

% Overview of the whole framework. 



\subsection{GPR Model Update}

% \subsubsection{Dataset Update}
In some previous literature, to facilitate the real-time implementation of the GPR in real-time applications like MPC, some approximation methods of GPR are adopted. However, these methods more or less lose the prediction accuracy of the GPR compared with the original GPR.
% , and some specific technology like choosing of inducing points are required, besides, their dataset is very small and not be able to be applied in a long track racing task, which is not very good.
In this paper, with the help of GPU, we adopt an efficient and general approximation of GPR based on Blackbox Matrix-Matrix multiplication (BBMM) \cite{gardner2018gpytorch}, which is able to support GPR model to be implemented in real-time with over 10,000 data points in GPR dataset while keeping almost the same prediction accuracy with original GPR.
Thus in our implementation, we augment our GPR dataset by stacking the data in each iteration to formulate our new GPR dataset.
The dataset $\mathcal{D}$ after $i$ th iteration is updated as

\begin{equation}
    \begin{split}
     \mb{Y}^i &= [\mb{Y}_0; \mb{Y}_1; \mb{Y}_2;\dots; \mb{Y}_i] \\
     \mb{Z}^i &= [\mb{Z}_0; \mb{Z}_1; \mb{Z}_2;\dots; \mb{Z}_i] \\
    \end{split}
\end{equation}
where $\mb{Y}^i$ and $\mb{Z}^i$ are the updated output and input dataset after $i$ th iteration,
$\mb{Y}_i$ and $\mb{Z}_i$ are the new output and input data collected in $i$ th iteration, where similar to $\mb{Y}_i$, input dataset $\mb{Z}$ is defined as $\mb{Z}= [\mb{z}^\top_1; \dots; \mb{z}^\top_m ] \in \mathbb{R}^{m \times n_f}$.

% \red{chagne simulation to experiment}

==> sections/metric_archive.tex <==
\subsection{Metric}
Based on the experimental setting that we stated above, in this subsection, we show the result that we obtain from the experiment. 
To better evaluate the performance of our proposed algorithm, here we list several metrics that we for the comparison
\begin{enumerate}
\item  Lap time: The time planned by the trajectory planner and actual lap time result by
tracking given trajectory.
% the racing vehicle to finish one loop tracking of the given trajectory
The time difference between planned trajectory and actual lap time result is also calculated to measure the model accuracy.

\item Model Error: 
Model error is the error between the true state and predict state. 
% Since we use different models in planning and MPC, therefore, 
Here we define the model errors with and without GPR error compensation in planning and MPC respectively as
\begin{itemize}
\item Planning:
\begin{equation}
\mb{e}^{plan} =  \frac{1}{N}\sum^{N}_{k= 0}||\dot{\mb{x}}_k^{real} - f(\mb{x}_k,\mb{u}_k)|| 
\end{equation}

\begin{equation}
\mb{e}^{plan}_{GPR} =  \frac{1}{N}\sum^{N}_{k= 0}||\dot{\mb{x}}_{k}^{real} - (f(\mb{x}_{k},\mb{u_{k}}) + \boldsymbol{\mu}^{plan}(\mb{z}_k))||
\end{equation}

\item MPC:
\begin{equation}
 \mb{e}^{MPC}=  \frac{1}{N}\sum^{N}_{k= 0}||\mb{x}_{k+1}^{real} 
% - (\mb{A}_{k} \mb{x}_{k}+\mb{B}_{k} \mb{u}_{k}) 
 % \mb{y}_k = \mb{x}_{k+1} 
 - (\mb{A}_{k} \mb{x}_{k}+\mb{B}_{k} \mb{u}_{k}+\mb{D}_{k})|| 
% \red{+ \boldsymbol{\mu}^{MPC?}(\mb{z}_k) }
\end{equation}

\begin{equation}
\begin{aligned}
 \mb{e}^{MPC}_{GPR}=  \frac{1}{N}\sum^{N}_{k= 0}||\mb{x}_{k+1}^{real}  
 - (\mb{A}_{k} \mb{x}_{k}+\mb{B}_{k} \mb{u}_{k}\\
 +\mb{D}_{k}+\boldsymbol{\mu}^{MPC}(\mb{z}_k)) ||
% \red{+ \boldsymbol{\mu}^{MPC?}(\mb{z}_k) }
\end{aligned}
\end{equation}
\end{itemize}

\item Tracking error: we use three tracking errors to evaluate the tracking performance of the given methods:

\begin{itemize}

    \item  $e^{\mu}_y$: mean lateral distance to the reference trajectory 
    \begin{equation}
        e^{\mu}_y = \frac{1}{N}\sum^{N}_{k= 0}| e_{y,k}|
    \end{equation}
    
    \item  $e^{\mu}_{vel}$: mean absolute error of the vehicle velocity compared to the reference trajectory
    \begin{equation}
        e^{\mu}_{vel} = \frac{1}{N}\sum^{N}_{k= 0}| V^{ref}_{x,k} - V^{real}_{x,k} |
    \end{equation}

    \item  $e^{\mu}_{heading}$: mean absolute error of the vehicle heading compared to the reference trajectory.

    \begin{equation}
    e^{\mu}_{heading} = \frac{1}{N}\sum^{N}_{k= 0}| e_{\psi,k}
    % + \beta_{i}
    |
    \end{equation}
    % \begin{equation}
    %     \beta_{i} =  \text{arctan}(\frac{V_{y,i}}{V_{x,i}})
    % \end{equation}
\end{itemize}

\item Number of Collisions $T_{collision}$: Times that the vehicle collides with the track wall in one-loop tracking experiment. 



\end{enumerate}


% We quantify the learning performance by comparing the average 2-norm of the model error in each lap w.r.t. the nominal model, i.e. 

% \red{Velocity profile and error figure
% G-G diagram
% \subsubsection{Case Study 1}
% \\
% az Compensate}
% \subsubsection{Case Study 1}
% Mazad Demio
% Vy Overestimate

==> sections/planning_and_control.tex <==
\section{Learning-based Trajectory Planning and Control Algorithms}\label{Sec:Plan_MPC}
% \blue{In a more general setting, we implement our controller and planner based on our previous work.}

In this section, we detail the planning and control modules that exploit our \textit{iterative, double GPR} method to compensate for modeling error and improve planning and tracking performance for autonomous racing. We employ GPR to provide two error compensation models; we then use these models in two modules: a 1) time-optimal trajectory planner and a 2) reference-tracking model predictive controller (MPC). In the following subsections, we first detail the planning and control frameworks, then describe the \textit{double-GPR} based modeling error compensation for both planning and control, and then describe the \textit{iterative} process for adapting the compensation model based on planning and control results.

\vspace{-1mm}
\subsection{Time-Optimal Trajectory Planning}\label{Sec:TrajPlan}
\vspace{-3mm}
We aim to plan a trajectory by directing solving a motion planning optimization problem to minimize the lap time, $T$, which can yield competitive racing results \cite{ourpriorwork}. Similarly, we adopt a close approximation of the minimum lap time objective that is derived by transforming the integral over the trajectory's horizon in \textit{time} to an integral in the \textit{spatial domain}~\cite{kapania2016sequential, ourpriorwork}. We likewise find a feasible initial guess by minimizing the curvature of a racing path and determining a feasible velocity for the path to reduce the potential for falling into suboptimal local optima. We summarize the minimum time objective here:
\begin{subequations}
\begin{align}
    \min_{\{\mb{x}_i\}_{i=1}^N,\{\mb{u}_{i}\}_{i=1}^N} \sum_{k=1}^{N} & \frac{\left(1-\kappa_k \ e_{y, k}\right) \Delta s_k}{V_{x, k} \cos \left(e_{\psi, k}\right)-V_{y, k} \sin \left(e_{\psi, k}\right)} \label{Equ:TimeObj} \\
    \mathrm{ s.t. } \quad \mb{x}_{k+1} & = \mb{x}_{k} + f(\mb{x}_{k},\mb{u}_{k}) \Delta t, \label{Equ:TimeObj_constr1}\\
    \mb{x}_{1} & =\mb{x}_{N}, \label{Equ:TimeObj_constr2}\\
    w_{r,k} & \leq e_{y,k} \leq w_{l,k}, \label{Equ:TimeObj_constr3}\\
    \delta_{\min,k } & \leq \delta_k \leq \delta_{\max,k }. \label{Equ:TimeObj_constr4}
\end{align}
\end{subequations}

In this motion planning problem, the constraints \eqref{Equ:TimeObj_constr2}, \eqref{Equ:TimeObj_constr3}, and \eqref{Equ:TimeObj_constr4} respectively ensure the state starts and ends at the same point, the vehicle remains within the track width on the left $w_{l,k}$ and right $w_{r,k}$, and the steering angle remains in the allowable range. The equality constraint \eqref{Equ:TimeObj_constr1} enforces that the states obey the vehicle model (\ref{equ:model_summary}). Since the time-optimal trajectory is constrained to remain feasible to the model, an accurate model is critical to result in a trajectory that is not only feasible, but is actually optimal for the racing environment.

\subsection{Learning-Based Model for Trajectory Planning}\label{Sec:gpr_plan}
\vspace{-3mm}
Since modeling errors can lead to suboptimal and infeasible planned trajectories, we augment the time-optimal trajectory optimization problem with a data-driven modeling error compensation term using GPR. In particular, in the modeling constraint \eqref{Equ:TimeObj_constr2}, we replace $f(\cdot, \cdot)$ with a compensated dynamic model for planning, $f_{{plan}}(\cdot, \cdot)$:
\begin{equation} \label{equ:plan_gpr}
     f_{{plan}}(\mb{x}_k,\mb{u}_k) = f(\mb{x}_k,\mb{u}_k) + \boldsymbol{\mu}^{plan}(\mb{z}_{plan}(\hat{\mb{x}}_k, \hat{\mb{u}}_k)),
\end{equation}
where $\boldsymbol{\mu}^{plan}$ is the mean of the error-compensating GPR model:
\begin{equation}\label{equ:plan_gpr_model}
\begin{aligned}
\mb{g}^{plan}(\mb{z})\sim 
\mathcal{N}(\boldsymbol{\mu}^{plan}(\mb{z}), \mb{\Sigma}^{plan}(\mb{z})).
\end{aligned}
\end{equation}
Similar to \cite{hewing2018cautious}, we restrict $\boldsymbol{\mu}^{plan}$ to only compensate a select number of states, namely $\dot{V_y}$ and $\ddot{\psi}$ since they have the most significant nominal modeling error; therefore, $\boldsymbol{\mu}^{plan}=\left[0;\mu^{plan}_{\dot{V_y}};\mu^{plan}_{\ddot{\psi}};0;0;0\right]^\intercal$.

The feature mapping function $\mb{z}_{plan}(\cdot,\cdot): \mathbb{R}^{n_s}, \mathbb{R}^{n_u}\rightarrow \mathbb{R}^{n_f} $ maps the state vector of dimension $n_s$ and the control action vector of dimension $n_u$ to the feature vector. To find an informative set of features, we design several candidate features and determine which features to include by analyzing the correlation coefficients between state errors and candidate features, and select the candidates that have the highest correlation with the state error as our features, as described in Section \ref{subsec:state_feature_select}. It is worth noting that the compensation term is defined with respect to a constant nominal state vector $\hat{\mb{x}}_k$ and a nominal control action vector $\hat{\mb{u}}_k$ rather than the actual $\mb{x}_k$ and $\mb{u}_k$, so that the GPR model is not directly embedded into the optimization problem. Instead, we just use the GPR model to predict a constant compensation term based on the nominal value. In planning, we set the nominal state and action vectors as the solution from the last iteration of time-optimal optimization~\cite{ourpriorwork}. 

Using \eqref{equ:plan_gpr}, the GPR model is combined with the nominal model $f(\cdot, \cdot)$ to compensate for modeling error with respect to the observed dataset. In particular, the dataset $\mathcal{D}^{plan}$ for the GPR model \eqref{equ:plan_gpr_model} consists of the observed states and actions, $\mb{x}_k$ and $\mb{u}_k$, and the output data point, $\mb{y}^{plan}_k$, defined as
\begin{equation}\label{equ:dtp_plan}
    \mb{y}^{plan}_k = \dot{\mb{x}}_k - f(\mb{x}_k,\mb{u}_k),
\end{equation}
where $\dot{\mb{x}}_k$ is the derivative of the observed state $\mb{x}_k$. 
% Here we also define the state error in planning $\mb{e}^{plan}$ is the same with $\mb{y}^{plan}_k$ as $\mb{e}^{plan} = \mb{y}^{plan}_k $.

\subsection{MPC Tracking Controller}
\vspace{-3mm}
\label{Sec:Controller}
A reference trajectory is provided by the time-optimal planner (Section \ref{Sec:TrajPlan}) with planning modeling error compensation (Section \ref{Sec:gpr_plan}).
We now introduce the MPC controller that tracks this reference trajectory.

Following our prior work~\cite{ourpriorwork}, we adopt a racing MPC with coupled longitudinal and lateral vehicle models that aims to reduce the tracking error between the actual vehicle state and the reference trajectory. The tracking objective and constraints are as follows:
\begin{subequations}\label{Equ:MPCCons}
\begin{align} 
\min_{\{\mb{x}_k\}_{k=1}^{N_p},\{\mb{u}_{k}\}_{k=1}^{N_{p-1}}} &
\sum_{k=1}^{N_{p}} \|\mb{x}_{k}-\mb{x}_{k}^{\mathrm{ref}}\|^{2}_{w_\mb{x}}+w_{\dot{\delta}} \Delta{\delta}_{k}^{2} \label{Eqn:MPCObj} \\
\mathrm{s.t.} \quad &\mb{x}_{k+1}=A_{k} \mb{x}_{k}+B_{k} \mb{u}_{k}+D_{k} \label{Eqn:MPCConstr1}\\
        & w_{r,k} \leq e_{y,k} \leq w_{l,k} \label{Eqn:MPCConstr2}\\
& u_{\min,k} \leq u_k \leq u_{\max,k}, \label{Eqn:MPCConstr3}
\end{align}
\end{subequations}
where $N_p$ is the prediction horizon of MPC. The objective function \eqref{Eqn:MPCObj} reduces the error between each of the states, with a weight corresponding to each element of the weight vector $w_\mb{x}\in \mathbb{R}^{n_s}$ with the dimension of $n_s$ same as the state $\mb{x}_k$, and regularization with weight $w_{\dot{\delta}}$ on the finite difference of steering angle to reduce rapid changes in steering angle. The term $\Delta{\delta}_k$ is defined as $\Delta{\delta}_k=\delta_k - \delta_{k-1}$. Constraints \eqref{Eqn:MPCConstr2} and \eqref{Eqn:MPCConstr3} are analogous to \eqref{Equ:TimeObj_constr3} and \eqref{Equ:TimeObj_constr4}, respectively. Unlike the nonlinear model employed by the trajectory planner, the MPC replaces constraint \eqref{Equ:TimeObj_constr1} with a linearization of the model \eqref{Eqn:MPCConstr1} to ensure the problem can be solved in real-time as a quadratic program. 
The linear model is found by linearizing the model around a heuristic nominal trajectory, $\bar{\mb{x}}_k$, as in~\cite{ourpriorwork}.

\subsection{Learning-Based Model for Control}\label{subsec:MPC_learning}
\vspace{-3mm}
The MPC in Section \ref{Sec:Controller} finds the best control actions by optimizing the tracking problem with respect to the model constraint \eqref{Eqn:MPCConstr1}. However, the control actions may not actually be optimal if \eqref{Eqn:MPCConstr1} does not accurately model the system. We therefore introduce an error compensation term in the MPC vehicle model constraint \eqref{Eqn:MPCConstr1} as:
\begin{equation}
    % \text { s.t. } \quad 
    \mb{x}_{k+1}=\mb{A}_{k} \mb{x}_{k}+\mb{B}_{k} \mb{u}_{k}+\mb{D}_{k} + \boldsymbol{\mu}^{MPC}(\mb{z}_k(\bar{\mb{x}}_k, \bar{\mb{u}}_k)), 
\end{equation}
where $\boldsymbol{\mu}^{MPC}$ is the mean of the GPR error model 
\begin{equation}
\begin{aligned}
\mb{g}^{MPC}(\mb{z})\sim 
\mathcal{N}\left(\boldsymbol{\mu}^{MPC}(\mb{z}), \mb{\Sigma}^{MPC}(\mb{z})\right).
\end{aligned}
\end{equation}
Similar to the GPR compensation function in planning, we restrict $\boldsymbol{\mu}^{plan}$ to only compensate $\dot{V_y}$ and $\ddot{\psi}$; therefore, $\boldsymbol{\mu}^{MPC} =\left[0;\mu^{plan}_{V_y};\mu^{MPC}_{\dot{\psi}};0;0;0\right]$. Also, we define a similar feature mapping function $\mb{z}_{MPC}(\cdot,\cdot): \mathbb{R}^{n_s}\times \mathbb{R}^{n_u}\rightarrow \mathbb{R}^{n_f}$. Similar to the case in planning, the compensation term is defined with respect to nominal state and action vectors. Here the nominal state and action vectors are chosen as the ones used for model linearization in the last subsection. 

To fit the GPR compensation function, we constructed a dataset $\mathcal{D}^{MPC}$ from the trajectories collected online. For each observed state $\mb{x}_{k+1}$, the output data point $\mb{y}^{MPC}_k$ in the dataset $\mathcal{D}^{MPC}$ is calculated as
\begin{equation}\label{equ:dtp_mpc}
\mb{y}^{MPC}_k = \mb{x}_{k+1} - (\mb{A}_{k} \mb{x}_{k}+\mb{B}_{k} \mb{u}_{k}+\mb{D}_{k}).
\end{equation}
% Similarly, we define the state error of MPC model $\mb{e}^{MPC}$ is the same with $\mb{y}^{MPC}_k$ as $\mb{e}^{MPC} = \mb{y}^{MPC}_k$.

\subsection{Iterative GPR Model Update Framework}\label{subsec:framework}
\vspace{-3mm}
So far we have detailed the trajectory planner and controller, each with corresponding error compensation functions using GPR. We now describe an iterative data collection scheme that ensures the GPR compensation functions are representative of the critical data regions for racing. The iterative framework is shown in Fig. \ref{Fig:framework}.
First in iteration 0, without exploiting GPR-based modeling error compensation, we plan a curvature-optimal trajectory~\cite{ourpriorwork} (\textbf{Step (1.1)}) and use the nominal MPC controller (Section \ref{Sec:Controller}) to track that trajectory (\textbf{Step (2)}) to collect data. After obtaining the initial dataset in the 0th iteration, we use it to build the initial GPR error compensation models (\textbf{Step (3)}) and apply them in the time-optimal trajectory planning (\textbf{Step (1.2)}) and subsequently MPC tracking (\textbf{Step (2)}). The closed-loop trajectories are added to the datasets for GPR. We use the augmented dataset to update our GPR model (\textbf{Step (3)}) and iteratively repeat \textbf{Step (1.2)}, \textbf{(2)}, and \textbf{(3)}.  Namely, The dataset $\mathcal{D}$ after $i^\text{th}$ iteration is updated as
\begin{equation}\label{eq:dataset}
    \begin{split}
     \mb{Y}^i &= [\mb{Y}_0; \mb{Y}_1; \mb{Y}_2;\dots; \mb{Y}_i] \\
     \mb{Z}^i &= [\mb{Z}_0; \mb{Z}_1; \mb{Z}_2;\dots; \mb{Z}_i] \\
    \end{split}
\end{equation}
where $\mb{Y}^i$ and $\mb{Z}^i$ are the updated output and input dataset after the $i^\text{th}$ iteration, $\mb{Y}_i$ and $\mb{Z}_i$ are the new output and input data collected in the $i^\text{th}$ iteration.  
% \blue{While maintaining a large number of data in GP dataset, we have difficulty doing online updating the GPR model.}

This iterative framework allows us to continuously update our GPR models for both planning and control using the most recent and historical data; this leads to improved modeling accuracy in both planning and control, and therefore improves the overall performance of the planning-control framework. It is worth noting that we choose to track the curvature-optimal trajectory (as opposed to a time-optimal trajectory) in iteration 0, because the data collected by tracking this alternative reference enriches data diversity, which was shown in our experiments to improve the prediction performance of the models. 
\blue{
% Besides,
% in order to ensure prediction accuracy for our long racing track,
% we require a GPR dataset containing over 10k data points. 
% However, managing such a large amount of data poses a challenge for performing online dataset update to the GPR model.
% Therefore, we opt for this loop-wise dataset updating rather than real-time updates to update our GPR model.
% Additionally, to speed up the optimization process of the parameters in GPR models, we randomly select 4000 data points in the GPR model dataset for parameter updating. If the dataset has less than 4000 data points, we use the whole dataset to update the parameters. The optimization of the parameters is carried out following \eqref{para_optm_func}.
% Eventually, for a GPR model with 19820 data points, we can finish optimizing to get a set of usable parameters within 130s.
To ensure prediction accuracy on our long racing track, we need a GPR dataset with over 10k data points. Managing such a large amount of data for online updates poses a challenge, so we update the dataset in loops instead of real-time. We randomly select 4000 data points to optimize parameters in the GPR model, or the entire dataset if it has fewer than 4000 points. Parameter optimization is done using \eqref{para_optm_func}. With 19820 data points, we can obtain usable parameters in 130s.
}



\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{fig/framework2.png}
    \caption{Iterative, double-GPR planning and control framework. \textbf{(1.1)}: At the $0^\text{th}$ iteration, curvature-optimal trajectory planning~\cite{ourpriorwork} without GPR error compensation; \textbf{(1.2)}: After $1^\text{st}$ iteration, time-optimal trajectory planning with GPR error compensation; \textbf{(2)}: Trajectory tracking GPR error compensation in MPC;\;\textbf{(3)}: Update of GPR error compensation models with tracking data.}\label{Fig:framework}
\end{figure}
\vspace{-3mm}
% Overview of the whole framework. 

% \red{chagne simulation to experiment}
